Essentials of Parallel Graph Analytics

We identify the graph data structure, frontiers, operators, an iterative loop structure, and convergence conditions as essential components of graph analytics systems based on the native-graph approach. Using these essential components, we propose an abstraction that captures all the significant programming models within graph analytics, such as bulk-synchronous, asynchronous, shared-memory, message-passing, and push vs. pull traversals. Finally, we demonstrate the power of our abstraction with an elegant modern C++ implementation of single-source shortest path and its required components.

==> tex/acknowledgement.tex <==
\section*{Acknowledgment}
\label{sec:acknowledgment}

\osama{??}

==> tex/case-study.tex <==
\section{Case-Study: Single-Source Shortest Paths}
\label{sec:case-study}
% A graph $G=(V,E)$ is comprised of $V$, set of all vertices, and $E$, set of all edges, where $E \subseteq V \times V$. 

The method we adapt for identifying key components of parallel data-centric graph analytics is to analyze traditional textbook approach solving a graph algorithm, such as Single-Source Shortest Paths (SSSP). The goal of this case study is to provide a simple implemention of SSSP, and then highlight the areas that can be parallelized. We can then extrapolate the essential components that generalize to other graph algorithms.

In this case study, we will be looking at \alg{Dijkstra's algorithm}. Given a weighted, directed graph $G=(V,E)$, with weights mapped to edges with the function $\omega : E \rightarrow {I\!R}$. Weight of any given path $p$ is the sum of the weights of its constituent edges. The goal of shortest-paths problems is to define a \alg{shortest path}, $\omega(p)$, for which the shotest-path weight $\delta(u, v)$ from $u$ (source-vertex) to $v$ (destination-vertex) is:~\cite{CLRS:2005:ITA} 

\begin{equation}
    \delta(u,v)=
    \begin{cases}
        \textbf{min}\{\omega(p) : u \rightarrow v\}, & \text{if a path exists from $u$ to $v$} \\
        \infty,                                      & \text{otherwise}
    \end{cases}
\end{equation}

\input{tex/textbook}

==> tex/components.tex <==
\section{Essentials of Data-Parallel Graph Analytics}
\label{sec:essentials}
% After having explored the textbook pseudocode, we can now summarize the essential components of the algorithm that we believe are important beyond just SSSP, to the data-centric parallel abstraction of graph analytics.
We identify the key insights from the case study in Section~\ref{sec:case-study}, building up the essential components of parallel data-centric graph analytics. We argue that the following components are significant to all underlying programming models, such as bulksynchronous (BSP) or asynchronous (AP) programming models (survey by McCune et al.~\cite{McCune:2015:TLA}), and allow for powerful expressive language for data-centric graph algorithms. We build the future of data-centric graph analytics on the same fundamental four pillars of TLAV frameworks surveyed by McCune, Weninger and Madey~\cite{McCune:2015:TLA}:

\begin{itemize}
    \item \textbf{Timing} Scheduling for execution: Synchronous, Asynchrnous, and Hybrid.
    \item \textbf{Communication} Communication model for data parallelism: Shared Memory and Message Passing.
    \item \textbf{Execution Model} Implementation of program execution and data flow: Vertex, Edge Programs and Push vs. Pull.
    \item \textbf{Partition} Graph partitioning and storage for parallel execution: Distributed, Streaming, Vertex Cuts and more.
\end{itemize}

This article will only cover data-centric parallel graph analytics using the bulk-synchronous and shared memory programming model approach, but we will identify where certain components can be extended to use an asynchronous model as well.

\subsection{Graph representation (as vertices and edges)} Although not explicitly mentioned in the pseudocode in the previous section, the graph representation is one of the fundamental components of data-centric graph analytics. In the pseudocodes described in Section~\ref{sec:textbook-sssp}, the graph is directly represented as a set of vertices with edges representing the connection among those vertices. And all of the implementations directly operate on either the vertex or the edge itself, or the data associated with the vertex or edge (for example, distances or predecessors).

The duality of graphs and sparse matrices can be exploited even in a data-centric graph analytics model. The underlying graph data structure can be expressed as common sparse matrix formats such as compressed-sparse row (CSR), compressed-sparse column (CSC) or an adjacency list. Sparse-matrix representations make for great graph representations due to the nature of storing really large graphs in a resonable amount of space. Contrary to a sparse matrix formats, storing a graph in a dense matrix representation will require considerably more memory. At a higher level, the user can query the graph data structure with only vertex and edge indices/iterators.  Listing~\ref{lst:graph-representation} shows one example of a graph internally represented as a sparse matrix, but queued with a data-centric API.

\begin{listing}[h]
    \caption{An example of requesting data from a sparse-matrix representation (CSR) with a data-centric API.\label{lst:graph-representation}}
    \begin{minted}[
        fontsize=\footnotesize,
        autogobble, breaklines]{c++}
        #include <vector>
        // Compressed-Sparse Row (CSR) matrix.
        struct csr_t {
            int rows;
            int cols;
            std::vector<int> row_offsets;
            std::vector<int> column_indices;
            std::vector<float> values;
        };

        struct graph_t : public csr_t {
            // Get edge weight for a given edge.
            float get_edge_weight(int const& e) {
                return values[e];
            }
        };
    \end{minted}
\end{listing}

\subsection{An active set of vertices or edges} In the data-centric model, an active set of vertices or edges is often referred to as the ``frontier'', containing the vertices/edges that are being processed in the algorithm. In the textbook SSSP pseudocode (Section~\ref{sec:textbook-sssp}), the frontier is represented as a min-priority queue. However, like graphs, a frontier can be represented in many different underlying representations as well. A sparse-frontier can simply be represented as a vector of active vertex or edge indices. A dense frontier can be represented as a boolean array, where each element is true if the corresponding vertex or edge is active.

Depending on the scheduling and communication model, these frontier representations can be partitioned or be streamed to the compute units for processing. For a bulk-synchrnous programming model with shared memory communication, the frontier can simply be stored in the shared memory (like the graph), and each element within the frontier can be processed in parallel. After each processing step, the synchronization step can be performed. In listing~\ref{lst:frontier}, we show how a sparse frontier can be implemented.

\begin{listing}[h]
    \caption{Sparse frontier of active vertices represented as a simple vector from C++ standard library.\label{lst:frontier}}
    \begin{minted}[
        fontsize=\footnotesize,
        autogobble, breaklines]{c++}
        #include <vector>
        struct frontier_t {
            // Underlying representation of frontier.
            std::vector<int> active_vertices;

            // Get the number of active vertices.
            int size() {
                return active_vertices.size();
            }
            // Get the active vertex at a given index.
            int get_active_vertex(int const& i) {
                return active_vertices[i];
            }
            // Add a vertex to the frontier.
            void add_vertex(int const& v) {
                active_vertices.push_back(v);
            }
        };
    \end{minted}
\end{listing}

\subsection{Operations on the active set} Operations on the active set are the expansion, contraction or transformations that are performed on the frontier, the active working set. These operations are the most fundamental component of any data-centric graph analytics, and are often where the fine-grained parallelism is abundant and explored in many different underlying abstractions (such as BSP). In the textbook SSSP pseudocode, the operation that is occuring is a traversal where for each vertex $v$ in the adjacency list of vertex $u$, a relaxation condition is applied, and this process happens for every vertex in the frontier.

%A high-performance graph analytics implementation relies on efficient parallel operators that transform, expand or contract the frontiers or graphs. This is where bulk of optimizations can be introduced, such as utilizing data-parallelism.

Continuing the bulk-synchronous programming with shared memory example from the previous sections, in listing~\ref{lst:operators} we show an example of how a prallel operator performing a traversal (frontier expansion) can be expressed using modern C++ programming language~(cite CPP).

\begin{listing}[h]
    \caption{Parallel neighbors expand, an operator derived from traditional textbook graph algorithm~\cite{CLRS:2005:ITA} implemented using modern C++. Note, due to use of execution policies, C++ 20 is required.\label{lst:operators}}
    \begin{minted}[
        fontsize=\footnotesize,
        autogobble, breaklines, obeytabs=false, tabsize=1]{c++}
        #include <algorithm>
        #include <execution>
        #include <mutex>
        // Neighbors expand implemented in C++ 20.
        template<typename expand_cond_t>
        frontier_t neighbors_expand(
            graph_t& g,
            frontier_t& f,
            expand_cond_t condition
        ) {
            std::mutex m;
            frontier_t output;
            auto expand = [&] (int const& v) {
                // For all edges of vertex v.
                for (auto e : g.get_edges(v)) {
                    auto n = g.get_dest_vertex(e);
                    auto w = g.get_edge_weight(e);
                    // If expand condition is
                    // true, add the neighbor into
                    // the output frontier.
                    if (condition(v, n, e, w)) {
                        std::lock_guard<std::mutex>
                            guard(m);
                        output.add_vertex(n);
                    }
                }
            };

            // For all active vertices in the
            // frontier, process in parallel.
            std::for_each(std::execution::par,
                f.active_vertices.begin(),
                f.active_vertices.end(),
                expand);

            // Return the new output frontier.
            return output;
        }
    \end{minted}
\end{listing}

\subsection{Initialization, convergence condition and the main loop}

\subsubsection{Initialization} A trivial, yet common step that appears in many algorithms is the preparation of initial data that often acts as the input to the algorithm. For data-centric graph analytics, this step is often the first step in the algorithm.
\subsubsection{Convergence Condition} The convergence condition is the condition that signals that the algorithm has completed. In the textbook SSSP pseudocode, the convergence condition is the condition that the frontier is empty.
\subsubsection{Main Loop} The main loop of the algorithm is the while-loop that iterates until a convergence condition has met. In a data-centric model, this is where the operators are organized and called to exploit the data-parallelism that exist within the algorithm. In the textbook SSSP pseudocode, the main loop is the while-loop that iterates until the frontier is empty.

Since the convergence condition, preparation of data and the main loop/organization of an algorithm is very specific to the algorithm itself, we follow the case-study presented in section~\ref{sec:case-study} to implement a parallel SSSP algorithm with the essential components (from section~\ref{sec:essentials}) in mind. The algorithm is implemented in listing~\ref{lst:sssp}.\footnote{Full implementation available here: https://bit.ly/3gFBYbz} The key insight to note is that using modern C++ and the data-centric parallel operators, we can reuse many of the same components (Listings~\ref{lst:graph-representation}-~\ref{lst:operators} are reusable) to implement other graph algorithms. For example, the \mintinline{cpp}{neighbors_expand} operator can be reused with a different C++ lambda (user-defined expand condition) to implement the parallel breadth-first search algorithm.

\begin{listing}[h]
    \caption{Parallel Single-Source Shortest Paths (SSSP) implemented in C++ using key components of data-centric graph analytics.\label{lst:sssp}}
    \begin{minted}[
        fontsize=\footnotesize,
        autogobble, breaklines, obeytabs=false, tabsize=1]{c++}
        std::vector<float> sssp(
            graph_t& g,
            int const& source
        ) {
            // Initialize data.
            std::vector<float> distances(g.get_num_vertices());
            for (auto v : g.get_vertices())
                distances[v] = std::numeric_limits<float>::max();
            distances[source] = 0;
            frontier_t f;
            f.add_vertex(source);

            while(f.size() != 0) {
                // Expand the frontier.
                f = neighbors_expand(g, f,
                // User-defined condition for SSSP.
                [&](int const& src,     // source
                    int const& dst,     // destination
                    int const& edge,    // edge
                    float const& weight // weight
                ) {
                    float new_d = distances[src] + weight;
                    // atomic::min atomically updates the distances array at dst with the minimum of new_d or its current value. And returns the old value. (eq: mutex updates)
                    float curr_d = atomic::min(&distances[dst], new_d);
                    return new_d < curr_d;
                });
            }
            return distances;
        }
    \end{minted}
\end{listing}


==> tex/expressing.tex <==
\section{Expressing Parallel Data-Centric Graph Analytics}
\label{sec:expressing}

The previous section summarizes key components required to implement data-centric graph analytics. In this section, we will use modern C++ programming language to provide a vision of how the key components can be materialized in practice to provide a high-performance implementation of graph algorithms. We build the future of data-centric graph analytics on the same fundamental four pillars of TLAV frameworks surveyed by McCune, Weninger and Madey~\cite{McCune:2015:TLA}:

\begin{itemize}
    \item \textbf{Timing} Scheduling for execution: Synchronous, Asynchrnous, and Hybrid.
    \item \textbf{Communication} Communication model for data parallelism: Shared Memory and Message Passing.
    \item \textbf{Execution Model} Implementation of program execution and data flow: Vertex, Edge Programs and Push vs. Pull.
    \item \textbf{Partition} Graph partitioning and storage for parallel execution: Distributed, Streaming, Vertex Cuts and more.
\end{itemize}

This article will only cover data-centric parallel graph analytics using the bulk-synchronous and shared memory programming model approach, but we will identify where certain components can be extended to use an asynchronous model as well.

\subsection{Graph representations}
The duality of graphs and sparse matrices can be exploited even in a data-centric graph analytics model. The underlying graph data structure can be expressed as common sparse matrix formats such as compressed-sparse row (CSR), compressed-sparse column (CSC) or an adjacency list. Sparse-matrix representations make for great graph representations due to the nature of storing really large graphs in a resonable amount of space. Contrary to a sparse matrix formats, storing a graph in a dense matrix representation will require considerably more memory. At a higher level, the user can query the graph data structure with only vertex and edge indices/iterators.  Listing~\ref{lst:graph-representation} shows one example of a graph internally represented as a sparse matrix, but queued with a data-centric API.

\begin{listing}[h]
    \caption{An example of requesting data from a sparse-matrix representation (CSR) with a data-centric API.\label{lst:graph-representation}}
    \begin{minted}[
        fontsize=\small,
        autogobble, breaklines]{c++}
        #include <vector>
        // Compressed-Sparse Row (CSR) matrix.
        struct csr_t {
            int rows;
            int cols;
            std::vector<int> row_offsets;
            std::vector<int> column_indices;
            std::vector<float> values;
        };

        struct graph_t : public csr_t {
            // Get edge weight for a given edge.
            float get_edge_weight(int const& e) {
                return values[e];
            }
        };
    \end{minted}
\end{listing}

\subsection{Frontier representations}
Like graphs, a frontier can be represented in many different underlying representations as well. A sparse-frontier can simply be represented as a vector of active vertex or edge indices. A dense frontier can be represented as a boolean array, where each element is true if the corresponding vertex or edge is active. Depending on the scheduling and communication model, these frontier representations can be partitioned or be streamed to the compute units for processing. For a bulk-synchrnous programming model with shared memory communication, the frontier can simply be stored in the shared memory (like the graph), and each element within the frontier can be processed in parallel. After each processing step, the synchronization step can be performed. In listing~\ref{lst:frontier}, we show how a sparse frontier can be implemented.

\begin{listing}[h]
    \caption{Sparse frontier of active vertices represented as a simple vector from C++ standard library.\label{lst:frontier}}
    \begin{minted}[
        fontsize=\small,
        autogobble, breaklines]{c++}
        #include <vector>
        struct frontier_t {
            // Underlying representation of frontier.
            std::vector<int> active_vertices;

            // Get the number of active vertices.
            int size() {
                return active_vertices.size();
            }
            // Get the active vertex at a given index.
            int get_active_vertex(int const& i) {
                return active_vertices[i];
            }
            // Add a vertex to the frontier.
            void add_vertex(int const& v) {
                active_vertices.push_back(v);
            }
        };
    \end{minted}
\end{listing}

\subsection{Parallel Operators}
A high-performance graph analytics implementation relies on efficient parallel operators that transform, expand or contract the frontiers or graphs. This is where bulk of optimizations can be introduced, such as utilizing data-parallelism. The operators can also be implemented with different execution models described in the McCune et al. survey~\cite{McCune:2015:TLA}. Following the bulk-synchronous programming with shared memory example from the previous sections, in listing~\ref{lst:operators} we show an example of how a prallel operator performing a traversal (frontier expansion) can be expressed using modern C++ programming language~(cite CPP).

\begin{listing}[h]
    \caption{Parallel neighbors expand, an operator derived from traditional textbook graph algorithm~\cite{CLRS:2005:ITA} implemented using modern C++. Note, due to use of execution policies, C++ 20 is required.\label{lst:operators}}
    \begin{minted}[
        fontsize=\small,
        autogobble, breaklines, obeytabs=false, tabsize=1]{c++}
        #include <algorithm>
        #include <execution>
        #include <mutex>
        // Neighbors expand implemented in C++ 20.
        template<typename expand_cond_t>
        frontier_t neighbors_expand(
            graph_t& g,
            frontier_t& f,
            expand_cond_t condition
        ) {
            std::mutex m;
            frontier_t output;
            auto expand = [=] (int const& v) {
                // For all edges of vertex v.
                for (auto e : g.get_edges(v)) {
                    auto n = g.get_dest_vertex(e);
                    auto w = g.get_edge_weight(e);
                    // If expand condition is
                    // true, add the neighbor into
                    // the output frontier.
                    if (condition(v, n, e, w)) {
                        std::lock_guard<std::mutex>
                            guard(m);
                        output.add_vertex(n);
                    }
                }
            };

            // For all active vertices in the
            // frontier, process in parallel.
            std::for_each(std::execution::par,
                f.active_vertices.begin(),
                f.active_vertices.end(),
                expand);

            // Return the new output frontier.
            return output;
        }
    \end{minted}
\end{listing}

\subsection{Example: Parallel Data-Centric SSSP}
Since the convergence condition, preparation of data and the main loop/organization of an algorithm is very specific to the algorithm itself, we follow the case-study presented in section~\ref{sec:case-study} to implement a parallel SSSP algorithm with the essential components (from section~\ref{sec:essentials}) in mind. The algorithm is implemented in listing~\ref{lst:sssp}. The key insight to note is that using modern C++ and the data-centric parallel operators, we can reuse many of the same components (Listings~\ref{lst:graph-representation}-~\ref{lst:operators} are reusable) to implement other graph algorithms. For example, the \mintinline{cpp}{neighbors_expand} operator can be reused with a different C++ lambda (user-defined expand condition) to implement the parallel breadth-first search algorithm.

\begin{listing}[h]
    \caption{Parallel Single-Source Shortest Paths (SSSP) implemented in C++ using key components of data-centric graph analytics.\label{lst:sssp}}
    \begin{minted}[
        fontsize=\small,
        autogobble, breaklines, obeytabs=false, tabsize=1]{c++}
        std::vector<float> sssp(
            graph_t& g,
            int const& source
        ) {
            // Initialize data.
            std::vector<float> distances(g.get_num_vertices());
            for (auto v : g.get_vertices())
                distances[v] = std::numeric_limits<float>::max();
            distances[source] = 0;
            frontier_t f;
            f.add_vertex(source);

            while(f.size() != 0) {
                // Expand the frontier.
                f = neighbors_expand(g, f,
                // User-defined condition for SSSP.
                [=](int const& src,     // source
                    int const& dst,     // destination
                    int const& edge,    // edge
                    float const& weight // weight
                ) {
                    float new_d = distances[src] + weight;
                    // atomic::min atomically updates the distances array at dst with the minimum of new_d or its current value. And returns the old value. (eq: mutex updates)
                    float curr_d = atomic::min(&distances[dst], new_d);
                    return new_d < curr_d;
                });
            }
            return distances;
        }
    \end{minted}
\end{listing}


==> tex/parallel.tex <==
\subsection{Gunrock: The Parallel CUDA/C++ Paradigm}
% Re-imagining Graph Algorithms for GPUs
% How does gunrock implement each of the three steps?
% Goal here will be to express the entire code in half a page!

Next we take a look at how the textbook SSSP algorithm, described in Section~\ref{sec:textbook-sssp}, can be transformed into a parallel SSSP algorithm implemented using Gunrock (Essentials). All code presented in the following listings is intended to be compilable using CUDA 11.5 (Ubuntu 18.04).

\subsubsection{Initialize}
Much like the textbook SSSP algorithm, the initialization step is intended to act as a pre-condition to the algorithm and is largely unchanged. We can use a helpful CUDA library called \lstinline{thrust} to declare the data and initialize it in parallel. Listing~\ref{lst:essentials-initialize} in line~6--25 shows the \lstinline{fill} functions are being executed in parallel (using the \lstinline{thrust::device} policy), which translates into a parallel loop, where each thread of the GPU is working on one element of the vector, and multiple threads are running in parallel. %cite thrust

\begin{listing}
\caption{Shows how we can write simple C++ code to execute on the GPU to initialize the respective data needed to implement parallel SSSP.\label{lst:essentials-initialize}}
\begin{minted}[
    fontsize=\footnotesize,
    obeytabs=true,
    tabsize=4,
    linenos,
    numbersep=-10pt]{c++}
    // Distance (d) and predecessor (pi) vectors.
    thrust::device_vector<float> d(num_vertices);
    thrust::device_vector<int> pi(num_vertices);
    int source = 0;

    // Initialize all distances to be infinity.
    thrust::fill(
        thrust::device, 
        d.begin(), 
        d.end(),
        std::numeric_limits<float>::max());

    // Except the distance to source node,
    // which is initialized to 0.
    thrust::fill(
        thrust::device, 
        d.begin() + source,
        d.begin() + source + 1, 
        0);

    // Set predecessors to be undefined.
    thrust::fill(
        thrust::device, 
        pi.begin(),
        pi.end(), 
        -1);
\end{minted}
\end{listing}

\subsubsection{Relax}
As explained in Section~\ref{sec:textbook-sssp}, relaxation step in SSSP consists of checking the path to a vertex by visiting its neighbors, and if a shorter path is found than the current path, the vertex is now updated to reflect the new distance and the new predecessor. How the relaxation step is launched and the condition is evaluated is where the most potential for writing an efficient and beautiful graph algorithm lies. In Gunrock's paradigm this is achieved using parallel operators, and the one we are interested in for our case-study is called the \lstinline{advance} operator. 

The \lstinline{advance} operator takes a set of vertices as an input, and visits all their neighboring vertices, generating a new set of these neighbors. The operator can be further extended by using C++ Lambda expressions (cite), which allows programmers to write a user-defined condition to apply to each of the source vertex, neighboring vertex, edge, weight tuple. Listing~\ref{lst:essentials-condition} shows one such condition, which evaluates if the current vertex distance is shorter than the new vertex distance in line~12, and that condition is used to determine if the neighbor is part of the next iteration's active vertex set in line~15.

\begin{listing}
    \caption{Shows a C++ Lambda expression extended with \lstinline{__device__} keyword (to allow it to run on the GPU) used for applying a user-defined condition on source, neighbor, edge, weight tupe.\label{lst:essentials-condition}}
    \begin{minted}[
        fontsize=\footnotesize,
        obeytabs=true,
        tabsize=4,
        linenos,
        numbersep=-10pt]{c++}
    auto shortest_path = [=] __device__(
        int const& v,   // ... source
        int const& u,   // neighbor
        int const& e,   // edge
        float const& w  // weight (tuple).
        ) -> bool {
        float v_d = d[v];
        float new_v_d = v_d + w;

        // Check if the destination node has 
        // been claimed as someone's child
        float recover_distance =
            math::atomic::min(&(d[u]), new_v_d);

        return (new_v_d < recover_distance);
    };
    \end{minted}
\end{listing}

\begin{listing}
    \caption{Shows how one can execute the relaxation step using an advance operator. Advance operator takes the graph, input and output frontiers and the GPU context on which the kernel should execute on as its input parameters.\label{lst:essentials-advance}}
    \begin{minted}[
        fontsize=\footnotesize,
        obeytabs=true,
        tabsize=4,
        linenos,
        numbersep=-10pt]{c++}
    // Execute the shortest_path lambda using advance.
    operators::advance::execute(
        G, E, shortest_path, context);
    \end{minted}
\end{listing}

Complete with Listings~\ref{lst:essentials-initialize}--\ref{lst:essentials-advance}, we have effectively implemented a variation of the textbook SSSP algorithm described in algorithm~\ref{alg:dijkstra}, all but the \lstinline{while}-loop from the pseudocode presented.

\subsubsection{Loop and Convergence Condition}
% Quick Notes:
\osama{Essentials loop is where advance operator or any other parallel operator gets implemented and called.
Users can extend and implement a virtual function called \lstinline{stop_condition}, which runs on every iteration and if it returns true the main-while loop ends.
For SSSP, that stop condition is simply if the frontier is empty.}

==> tex/performance.tex <==
\subsection{Performance Characteristics}
\osama{Performance analysis of parallel vs. sequential and maybe state-of-the-art for the GPUs.
I wonder if we can use GraphBLAS for CPU-code to make it a fair compairson, or some other equivalent high-performance CPU library.}

==> tex/textbook.tex <==
\subsection{Textbook SSSP Algorithm}
\label{sec:textbook-sssp}
% Sequential SSSP algorithm that clearly divides the problem into digestable parts.
Pseudocode for Dijkstra's algorithm as presented in ``Introduction to Algorithms'' by Cormen et al.~\cite{CLRS:2005:ITA} can be broken down into three individual steps:

\begin{enumerate}
    \item An initialization stage,
    \item Conditions applied on traversal (relaxation), and
    \item Main loop organization and condition for convergence of the algorithm.
\end{enumerate}

\subsubsection{Initialize}
\label{sec:textbook-sssp-initialize}
Acts as a pre-condition to the algorithm, setting up all the required data to be later processed in the main loop. In pseudocode~\ref{alg:initialize} we see an example of what an initialization step could look like for Dijkstra's SSSP. To set up the SSSP algorithm, we begin by setting all distances to infinity for all of the vertices in the graph except the source vertex, which is set to $0$. We also set all of the predecessors to be undefined, as these will be discovered as the algorithm processes. Note that this can be trivially updated to support parallelism since every distance and predecessor is set independently from the other. In a parallel variation of the pseudocode~\ref{alg:initialize}, we can envision the sequential for-each in line~2 can be updated to a parallel for-all that operates on all distances and predecessors concurrently.


\begin{algorithm}
    \floatname{algorithm}{}
    \caption{Initialize the distances to all vertices to be $\infty$ and the distance to the source to be $0$.\label{alg:initialize}}
    \begin{algorithmic}[1]
        \Function{initialize}{$G,s$}
        \ForEach{vertex $v \in G.V$} \Comment{Parallel: \textbf{for}}
        \State $v.d = \infty$
        \State $v.\pi = \text{NIL}$
        \EndFor
        \State $s.d = 0$
        \EndFunction
    \end{algorithmic}
\end{algorithm}


\subsubsection{Relax}
As the authors of ``Introduction to Algorithms'' describe, the process of relaxation is used in many graph algorithms and consists of testing a condition while visiting an edge $e$ consisting of vertices $u, v$. ~\cite{CLRS:2005:ITA} For SSSP, this condition happens to be proving the shortest path to vertex $v$ found so far by visiting vertex $u$ (see pseudocode ~\ref{alg:relax}). If this path happens to be the shortest, the distance and predecessor for vertex $v$ are updated. The key take-away from relaxation step is that the exact same condition may apply to many vertices during the life of the SSSP algorithm, and that the relaxation condition may differ from algorithm to algorithm. Therefore, when expressing the relaxation stage in our data-centric programming model, we need to be able to modify the condition to suit other graph algorithms.


\begin{algorithm}
    \floatname{algorithm}{}
    \caption{If the current distance of the vertex $v.d$ is greater than the sum of distance of the neighbor, $u.d$, and the edge weight, $\omega(u,v)$, then we have found a new minimum shortest-path estimate.\label{alg:relax}}
    \begin{algorithmic}[1]
        \Function{relax}{$u,v,\omega$}
        \If{$v.d > u.d + \omega(u, v)$}
        \State $v.d = u.d + \omega(u,v)$
        \State $v.\pi = u$
        \EndIf
        \EndFunction
    \end{algorithmic}
\end{algorithm}


\subsubsection{Loop and Convergence Condition}
The final component for Dijkstra's algorithm is described in pseudocode~\ref{alg:dijkstra}, which shows the required steps that are organized to successfully implement the complete algorithm: 

\begin{itemize}
    \item Line~2: We start by calling our initialization function described in section~\ref{sec:textbook-sssp-initialize} to set up the data structures.
    \item Line~3: The output set is defined to initially be an empty set.
    \item Line~4: We set up an active set of vertices to be processed, which is initially the set of all vertices in the graph.
    \item Line~5: Begins the main-loop, which is a while-loop that iterates until the active set is empty.
    \item Line~6--7: We select a vertex $u$ from the active set to be processed using the priority queue, and adds $u$ to the output set.
    \item Line~8--9: We perform a traversal on vertex $u$, visiting each neighbor $v$ and edge $e$ of $u$ and updating the distance and predecessor of $v$ if necessary (relax condition).
\end{itemize}
Important aspects to note from this section of the algorithm are 1) the need for an active set of vertices, 2) the for-loop traversing the neighbors of vertex $u$, which can be parallelized, and 3) the iterative nature of the algorithm and the convergence condition to signal that the algorithm has completed.

\begin{algorithm}
    \floatname{algorithm}{}
    \caption{Dijkstra's single-source shortest path algorithm for weighted, directed graphs with nonnegative weights. Where $S$ represents the output set and $Q$ is a priority-queue for active vertex set.\label{alg:dijkstra}}
    \begin{algorithmic}[1]
        \Function{dijkstra}{$G,\omega,s$}
        \State \Call{initialize}{$G, s$}
        \State $S = 0$
        \State $Q = G.V$
        \While{$Q\neq0$}
        \State $u = $ \Call{extract-min}{$Q$}
        \State $S = S \cup\{u\}$
        \ForEach{vertex $v \in G.Adj[u]$} \Comment{Parallel: \textbf{for}}
        \State \Call{relax}{$u,v,\omega$}
        \EndFor
        \EndWhile
        \EndFunction
    \end{algorithmic}
\end{algorithm}
